Thermally-induced microstructural evolution in nanoparticle-based CuO, WO$_3$ and CuO-WO$_3$ thin films for hydrogen gas sensing

This study systematically investigates the microstructural evolution of nanoparticle-based CuO, WO$_3$, and composite 'CuO-WO$_3$' thin films induced by their post-deposition annealing. The films were reactively deposited using a magnetron-based gas aggregation technique, with the composite films consisting of alternating monolayers of CuO and WO$_3$ nanoparticles. After deposition, the films were annealed in synthetic air at temperatures ranging from 200 to 400$^\circ$C and characterized using scanning electron microscopy, X-ray diffraction, Raman spectroscopy, and X-ray photoelectron spectroscopy. Annealing of the CuO films led to the most pronounced changes associated with a gradual enhancement of crystallinity accompanied by significant particle growth with increasing annealing temperature, while the WO$_3$ and CuO-WO$_3$ films were more thermally stable to crystallization and particle growth. Notably, at 400$^\circ$C, the CuO--WO$_3$ films crystallized into a novel $\gamma$-CuWO$_4$ phase. The annealed films were further evaluated for their gas-sensing performance upon H$_2$ exposure and the obtained results were analyzed in relation to film properties and the microstructural evolution induced by annealing.

==> BAK/XPS.tex <==
%CuO NPs%
%XPS measurements were performed to examine the structural evolution with increasing annealing temperature. Core-level spectra of O, Cu, and W were analyzed using Voigt and Voigt doublet functions. The Cu\,2p spectra for CuO NPs (Fig. \ref{fig XPS CuO}a) show a peak at 932.89\,eV, likely corresponding to a mixture of Cu$_2$O (932.18–932.5\,eV) and metallic Cu (932.63–932.7\,eV) \cite{Biesinger2010, chastain1995handbook}. However, based on the preparation process and as confirmed by the XRD results (Fig. \ref{fig:XRD 400C}a), the presence of pure Cu NPs is unlikely. The second peak at 934.33\,eV corresponds to CuO (933.6–933.8\,eV) \cite{Biesinger2010, chastain1995handbook}, indicating that Cu$_2$O NPs are oxidized to CuO at elevated temperatures. The peak at 935.67\,eV, attributed to Cu(OH)$_x$, decreases as temperature increases, confirmed by the O\,1s spectra (Fig. \ref{fig XPS CuO}b). Other features in the Cu\,2p spectra include typical satellite peaks of Cu$_2$O and Cu(OH)$_x$. The O\,1s spectra (Fig. \ref{fig XPS CuO}b) consist of three components: the first at 529.77\,eV, representing a mix of Cu$_2$O and CuO, the second at 531.23\,eV, corresponding to surface contamination such as Cu(OH)$_x$ and other hydroxides or carbonates, and the third at 532.07\,eV, likely due to adventitious organic compounds. With increase in temperature, the intensity of the contamination-related peaks (531.23\,eV and 532.07\,eV) decreases due to desorption, while that of the metallic oxide peaks increase, indicating oxygen saturation in Cu$_2$O and CuO NPs. This trend is consistent with the XRD results, showing strong peaks of m-CuO at elevated temperatures (Fig. \ref{fig:XRD 400C}a).

The XPS spectra of WO$_3$ NP films are shown in Fig. \ref{fig XPS WO3}. In the W\,4f spectra (Fig. \ref{fig XPS WO3}a) two components are identified: WO$_3$ at 35.84\,eV (consistent with literature values of 35.7\,eV \cite{SHPAK2007172} and 35.8\,eV \cite{chastain1995handbook}) and probably WO$_x$ at 34.38\,eV. Although WO$_2$ is unlikely, as it typically appears at lower binding energies around 32.8\,eV \cite{chastain1995handbook}, Khyzhun et al. have assigned similar peaks to substoichiometric WO$_x$ \cite{Khyzhun2002}. With increasing annealing temperature, although only a small decrease in the intensity of the WO$_x$ peak is observed, a significant shift of the WO$_3$ peak to lower binding energies is visible. This shift maybe due to the microstructural evolution and crystallization of WO$_3$ at 300\,$^{\circ}$C, as evidenced by XRD (Fig. \ref{fig:XRD 400C}b). A similar phenomenon was reported by Liu et al. when TiO$_2$ crystallized after annealing at 400\,$^{\circ}$C \cite{8325473}. Fig. \ref{fig XPS WO3}b shows the evolution of the O\,1s peak in WO$_3$ NPs. Similar to the W\,4f spectrum, the main peak at 530.82\,eV corresponds to the metallic oxides of WO$_3$, likely with a small amount of WO$_x$. This is consistent with the binding energy of WO$_3$ reported by Chastain \cite{chastain1995handbook} and Shpak \cite{SHPAK2007172} at 530.6\,eV. The other two peaks are attributed to surface contamination, likely in the form of hydroxides, carbonates, or other surface-bound species.


==> alternative_introduction.tex <==
\section{Introduction}

Nanomaterials have emerged as key components in a number of modern functional material applications because of their unique properties. Among these, nanoparticle-based materials stand out for their high surface area, tunable morphology, and exceptional reactivity, making them indispensable in fields such as medicine, electronics, environmental sensing, and energy storage. Specifically, in the realm of energy, nanoparticles (NPs) play a crucial role in hydrogen-related technologies. Hydrogen, as a clean and renewable energy carrier, holds promise for diverse applications. \cite{Manoharan2019, Muradov2008}. The development of safe and effective hydrogen technologies, among others, calls for reliable sensing technologies, which are essential for monitoring and regulating hydrogen concentrations across diverse applications.

The microstructure of the sensing material is crucial for achieving optimal gas sensing performance, as it directly influences the interactions between the sensing material and analytes \cite{Zhao2023}.  In addition, optimizing the dimensions and spatial arrangement of the individual building blocks (such as nanoparticles) within nanomaterials enhances their transducer function, facilitating the conversion of chemical interactions with analyte gases into measurable electrical signals \cite{Girolamo2009, Ghenadii}.

When dealing with NP-based material, the formation of 'necks' at the junctions among individual NPs heavily affects the conductivity of the percolation network within the material. Smaller 'necks' can dynamically 'close/open' in response to the formation of the depletion layer (DL), thereby modulating the material's electrical properties \cite{Jun2009}. Furthermore, combining different metal oxides to form heterojunctions at their interfaces can lead to even greater sensitivity to analytes, as these heterojunctions deepen the DL and amplify changes in conductivity \cite{Korotcenkov2017, Yang2021}.

Among various gas-sensing technologies, conductometric sensors have garnered significant attention due to their high sensitivity, rapid response, and cost-effectiveness \cite{Antonio2022, Joshi2018}. These sensors operate on the principle that the electrical conductivity of the sensing material changes in response to the presence of target gases (analytes), enabling their detection and quantification. Metal oxide semiconductors (MOS) are particularly renowned for their superior performance as conductometric sensors \cite{Goel2023, Nadargi2023}. In MOS-based sensors, gas molecules adsorb and desorb on the semiconductor surface, altering the carrier concentration near the surface, the so-called depletion layer (DL), and consequently changing the electrical properties of the material.

Given that the microstructure of NP-based films plays a crucial role in determining their gas-sensing performance, it is essential to consider how post-deposition thermal annealing can affect the microstructural evolution and further optimize the properties of these films. Thermal annealing not only promotes crystallinity but also induces changes in NP size, density of adsorption sites, film composition, and other microstructural features. Such modifications impact the formation of interparticle necks and surface interactions with target gases, ultimately affecting charge carrier dynamics and gas sensing efficiency. 

In this work, we investigate the influence of the thermal treatment on NP-based thin films synthesized using a magnetron-based gas-aggregation source (GAS). Nanoparticles produced by this method can be of many kinds; in this work, we investigated thin films based on metal-oxide-semiconductor (MOS) nanoparticles CuO and WO$_3$ and the films formed by their combination. The detailed multi-scale structural study (spanned from the atomic scale to the morphological one) is supplemented by measurements of sensing properties of synthesized structures with conscious attention to the relation of structure to sensing behavior. NPs produced by GAS have been studied for a few years now, but only a few publications are dedicated to their thermal evolution during annealing and even fewer when considering their percolating networks.

Our comprehensive multi-scale structural study spans from the atomic to the morphological scale. This analysis is complemented by measurements of the hydrogen gas sensing properties of the synthesized structures, with careful attention to the relationship between their structure and sensing behavior. Although GAS NPs have been studied over the past few years, only a limited number of publications have focused on their thermal evolution during annealing \cite{Hanková2023, Košutová2022}. Furthermore, even fewer studies have explored the impact of thermal treatment on their percolating networks.

Among various MOSs, single material CuO and WO$_3$ nanoparticles (NPs) have demonstrated excellent potential for gas sensing applications \cite{Steinhauer2021, Dong2020}. In our recent works \cite{Kumar2020, Kumar2021, Haviar2018}, we have shown that the sensing performance can be further enhanced by the synergistic combination of CuO NPs with a WO$_3$ thin film. This enhancement is attributed to the formation of nano-sized p-n heterojunctions between p-type CuO and n-type WO$_3$. These heterojunctions significantly improve sensor sensitivity by efficiently modulating charge carrier dynamics at the interface. Building on these findings, we optimized our deposition technique using a GAS for the one-step controlled synthesis of composite thin films consisting of alternating monolayers of CuO and WO$_3$ NPs \cite{Shaji2024}. This physical deposition technique enables the synthesis of various combinations of high-purity NPs with tunable size, composition, and morphology.


